Comparative Snippet Generation

We model product reviews to generate comparative responses consisting of positive and negative experiences regarding the product. Specifically, we generate a single-sentence, comparative response from a given positive and a negative opinion. We contribute the first dataset for this task of Comparative Snippet Generation from contrasting opinions regarding a product, and a performance analysis of a pre-trained BERT model to generate such snippets.

==> comments.orig.tex <==
ACL 2022 Workshop ECNLP Paper14 Reviewer n43E posted a new Official Review to ACL 2022 Workshop ECNLP Paper14 × 3  •  7 days ago
Authors create a dataset for the task of Comparative Snippet Generation from contrasting opinions regarding a product.
 Comparative Snippet Generation
Review:
The paper introduces a novel task of generating a comparative response showing positive and negative opinions using BERT based encoder decoder architecture.
Overall, this is a borderline paper, as the task is interesting and novel, but the presentation is lacking in motivation and there is a lack of novelty on the modeling side as well. In particular, the authors spend a bulk of the paper describing different experiments and results. The authors need to provide a clearer explanation of the motivation: why is answering this research question important or valuable? Has prior work suggested that this is something important or valuable to study? Specifically, it would have been nice for the work to more explicitly state their contribution, and where the novelty in their method lies in relation to the related work.

Rating: 6: Marginally above acceptance threshold
Confidence: 4: The reviewer is confident but not absolutely certain that the evaluation is correct
ACL 2022 Workshop ECNLP Paper14 Reviewer gUN5 posted a new Official Review to ACL 2022 Workshop ECNLP Paper14 × 3  •  12 days ago
A new dataset and preliminary experiment on comparative product reviews
 Comparative Snippet Generation
Review:
The paper “Comparative Snippet Generation“ aims at generating product reviews mixing good and bad features, e.g. “the tablet is cheap but pretty slow”. As part of the submission, the dataset created for the work will be released to the community.

The paper tackles a novel problem, whose business and industry importance is however not clear: why doing these snippets would be helpful at all? What metrics / industry / UX trend suggest that this is a worthwhile investigation? Novelty alone is a poor proxy for impact, especially if the research contribution itself is not general enough to be widely appealing to practitioners.

 Even not considering the strength of the motivation section, I find it hard to understand the reasoning behind the experiments. From the phrasing in section “Rule-based Response Generation” and below (“our next task is to generate a  dataset into the required format as shown in Table 4”, "We generate dataset in two phases and follow all the steps mentioned in the section”), it seems the dataset is mostly (or entirely) generated out of 7 templates, making it fairly easy for models to just learn those patterns. Moreover, the logic behind the experimental section is not entirely clear to me: “As shown in Table 5, recall 453 of model-based generations is high, 0.9876, yet 454 less than rule-based generation” - if rule-based generation is the gold standard to create the dataset, it doesn’t look like a sound comparison. Even the examples of generalization (“and has been generated 485 by fusing “however”, and “some users have also”) are fairly trivial for modern language models, and don’t seem to add value to the work, either practically (rule-based generation seems to be already good) or theoretically (given contemporary NLP, this result does not seem particularly interesting or general).

Overall, I think the most valuable contribution for the community could be the dataset itself: while it is clear that it has been built by combining off the shelf tools in a fairly straightforward way, datasets are still a very important part of the progress we make as a field. However, I would suggest authors to invest more time in building an even better, more varied dataset and to submit to, say, SIGIR eCOM data track, instead of presenting the work as a research paper.

I added some small notes below to help authors improve their submission, but for the reasons explained above I don’t think this paper should be accepted.

Formal notes:

The GitHub link (https://github.com/saurabhhssaurabh) breaks anonymity in the process. I didn’t count this mistake in my review, but I wish to point it out as i) a formal comment on the CFP rules, ii) a helpful suggestion for the authors.

Minor notes:

”E-commerce websites do provide functionality to compare products. These functionalities are template-based and compare products or services”. This generalization is a bit too strong: comparisons are not necessarily template-based and data extraction may actually play a big role in recommenders built with comparison in mind: for example, see last year’s SIGIR paper (https://arxiv.org/abs/2107.03256) as a ref.

“Due to the effectiveness 386 of the BERT model over Transformers for the text 387 generation tasks “. True as a general sentence, but need a reference.

Rating: 4: Ok but not good enough - rejection
Confidence: 4: The reviewer is confident but not absolutely certain that the evaluation is correct
